Fail2Progress: Learning from Real-World Robot Failures with Stein Variational Inference

Skill effect models for long-horizon manipulation tasks are prone to failures in conditions not covered by training data distributions. Therefore, enabling robots to reason about and learn from failures is necessary. We investigate the problem of efficiently generating a dataset targeted to observed failures. After fine-tuning a skill effect model on this dataset, we evaluate the extent to which the model can recover from failures and minimize future failures. We propose Fail2Progress, an approach that leverages Stein variational inference to generate multiple simulation environments in parallel, enabling efficient data sample generation similar to observed failures. Our method is capable of handling several challenging mobile manipulation tasks, including transporting multiple objects, organizing a constrained shelf, and tabletop organization. Through large-scale simulation and real-world experiments, we demonstrate that our approach excels at learning from failures across different numbers of objects. Furthermore, we show that Fail2Progress outperforms several baselines.

==> failures.tex <==
Consider a robot operating using a relational dynamics model $\rd$ trained on some dataset, \(\dataset\).
A user tasks the robot to achieve a goal, $\mathcal{G}$.
Given an initial observation, $O_0$, it's relational dynamics model, and the goal, the robot plans a skill sequence, $\SkillSeq$. In addition to the skill sequence itself the relational dynamics model predicts a sequence of expected relations, \(\mathcal{R}_{k}^{\prime}\) (i.e. symbolic states) that the robot will observe after executing each skill in its sequence for \(k=1,\ldots,H\).

The robot now begins executing its skills following the plan.
After each skill execution in the sequence the robot can observe the current scene, \(O_k\), and detect the current symbolic state as \(\hat{\mathcal{R}}_k\). When the observed relations, \(\hat{\mathcal{R}}_k\), don't match the predicted relations, \(\mathcal{R}_k^{\prime}\), the robot detects that it has failed to achieve the current subtask. We now consider the problem of learning from this failure instance to improve the relational dynamics model $\rd$. Note that if the robot does not precisely achieve the predicted geometric state (e.g. predicted  poses), but does achieve the correct relations, it does not consider it a failure. In such cases, the robot updates its continuous skill parameters conditioned on the current observation and continues executing the sequence.

In the case of a detected failure, the robot stores the associated failure event in order to learn from it.
We define a failure event to include the relevant observations, relations (i.e. symbolic-states), and skill associated with the failure: \(\fail = (O^{\fail}=O_k, \mathcal{R}^{\fail}=\mathcal{R}_k, \phi^{\fail}=\phi_k, \mathcal{R}^{\fail\prime}=\hat{\mathcal{R}}_{k+1})\)

==> overview_fig.tex <==
\setcounter{figure}{1}
\makeatletter
\let\@oldmaketitle\@maketitle%
\renewcommand{\@maketitle}{\@oldmaketitle%
  \begin{center}
    \centering
    \includegraphics[width=\textwidth]{figures/figure1_v7.pdf}
    \vspace{-15pt}
  \end{center}
\footnotesize{\textbf{Fig.~\thefigure:\label{fig:overview_figure}} \textbf{Overview of Failure Case Reasoning.} \textbf{Top}: Based on failure cases, our approach generates targeted, diverse simulation data in parallel to fine-tune the robot's model. 
  \textbf{Bottom}: The fine-tuned model successfully performs diverse long-horizon manipulation tasks in challenging real-world scenarios.}
  \medskip}
\makeatother
\shrinka
\maketitle
\shrinka
\thispagestyle{empty}
\pagestyle{empty}
